Classification As Decoder: Trading Flexibility For Control In Neural Dialogue

Generative seq2seq dialogue systems are trained to predict the next word in dialogues that have already occurred. They can learn from large unlabeled conversation datasets, build a deep understanding of conversational context, and generate a wide variety of responses. This flexibility comes at the cost of control. Undesirable responses in the training data will be reproduced by the model at inference time, and longer generations often don't make sense. Instead of generating responses one word at a time, we train a classifier to choose from a predefined list of full responses. The classifier is trained on (conversation context, response class) pairs, where each response class is a noisily labeled group of interchangeable responses. At inference, we generate the exemplar response associated with the predicted response class. Experts can edit and improve these exemplar responses over time without retraining the classifier or invalidating old training data. Human evaluation of 775 unseen doctor/patient conversations shows that this tradeoff improves responses. Only 12% of our discriminative approach's responses are worse than the doctor's response in the same conversational context, compared to 18% for the generative model. A discriminative model trained without any manual labeling of response classes achieves equal performance to the generative model.

==> sections/clustering_anitha.tex <==
\subsubsection{Anitha's Automatically Cluster Similar Responses}

We denote the set of $N$ response messages by $\mathcal{R} = \{r_1, \cdots r_N\}$. 

The goal is to induce a clustering on $\mathcal{R}$ so that these clusters can serve as 
labels. For this purpose, we use agglomerative clustering - starting with treating each $r_i$ as  
as a separate cluster, the approach repeatedly merges them by using the following objective:
\begin{equation}
    [C_a,  C_b] = \argmax_{C_i,  C_j , i \neq j } A(C_i,  C_j)
\end{equation}

We next discuss our methodology for computing affinity (similarity) between pairs of responses, $r_i$ and $r_j$
\para \noindent
{\bf Similarity between responses}: We use a learned similarity function between pairs of input sentences. In particular, we 
use a BERT \citep{devlin2018bert} model finetuned on the task of Quora Question similarity task \cite{Wang_2018} so that:

Estimating the affinity of every pair of responses is an O($\mathcal{R}^2)$ operation and most pairs are likely to have negligible similarity. Therefore, we restrict computing similarities of $r_i$
to only responses that are within a neighborhood, $\mathcal{N}(r_j)$:
\begin{equation}
    affinity(r_i, r_j) = \begin{cases} p(similarity=1| r_i, r_j) , & \text{ if} r_i \in \mathcal{N}(r_j )  \\ 0  \textrm{  otherwise} \end{cases}, 
\label{eq:ce}
\end{equation}

\para \noindent
{\bf Inferring neighbors}: 
For each response message, $r_i$, Let $f_e(r_i)_{e=1}^{K}$ be $K$ different distributed deep representations of the message, obtained using 
pre-trained sentence encoders. In this paper, we used InferSent \citep{conneau-EtAl:2017:EMNLP2017}, the finetuned AWD-LSTM language model and the average Glove \citep{pennington2014glove} word vector for the response.
Then, we can compute the top nearest neighbors of a response message as the union of the nearest neigbors for each of these. In particular,
\TODO{fix notation here}
\begin{equation}
    \mathcal{N}(r_i ) = \bigcup_{f_e(r_i)} KNN(f_j(r_i), \mathcal{R}-r_i, 10)
\end{equation}
\TODO{discuss utility of using multiple encoders in terms of goodness of each method}



==> sections/clustering_v1.tex <==



\begin{enumerate}
\item \textbf{Automatically Cluster Similar Responses}
\begin{enumerate}
  \item We lower case, remove patient and doctor identifying information, and remove punctuation from all responses seen in the data. We consider only the preprocessed responses $R$ that occur more than once, to make subsequent steps computationally cheaper.
  %We consider only the 60,000 preprocessed responses (20\% of all responses) that occur more than once, to make subsequent steps computationally cheaper.
  \item Estimating the similarity of every pair of responses is an O($\mathcal{R}^2)$ operation and most pairs are likely to have negligible similarity. Therefore, we restrict computing similarities of $r_i$
to only responses that are within a semantic neighborhood. More specifically, we encode each response as a vector using three pretrained sentence encoders: InferSent \citep{conneau-EtAl:2017:EMNLP2017}, the finetuned AWD-LSTM language model, the average Glove \citep{pennington2014glove} word vector for the response, and the TFIDF weighted average of the Glove vectors. For each encoder, we take the 10 nearest neighbors for each response. 
 $$
CandidatePairs =  \bigcup_{j \in encoders, i \in R}(i, KNN(enc_{j, -}, enc_{j, i}, 10))
$$
   % This yields 1 million unique candidate pairs, roughly 17 per response. 
  \item  For each candidate pair, we run a supervised similarity model, BERT \citep{devlin2018bert} pretrained on Quora Question Pairs \citep{Wang_2018}, to predict the probability that each response pairs' members are semantically similar. We store the dissimilarity of each pair in a sparse distance matrix, with a distance of 1 (the maximum) if two responses were not blocked together. 
  $$
D_{i, j} =  
\begin{cases}
    (1 - ProbSimilar_{i,j}), & \text{if } (i,j) \in CandidatePairs\\
    1,              & \text{otherwise}
\end{cases}.
$$
  \item 
The last step is Agglomerative Clustering, on $D$,  where the distance between two responses is their predicted probability of dissimilarity or 1 if they were not generated as a candidate pair.  Merging requires complete linkage, which means that two clusters are only merged if all the responses in both clusters are >= 75\% similar to all responses in the other cluster. %After this step, we have 40,000 clusters.
$$
Cluster_{i} = AgglomerativeClustering(D,  distanceThreshold=0.25)
$$
\end{enumerate}
\item \textbf{Manually Merge Clusters into Response Classes}
\begin{enumerate} 
\item Create dataset containing (centroid text, \# occurences of cluster constituents), sorted by \# occurrences, 
where the centroid is the most frequently occurring response in the cluster.
\item For each row in the dataset, the labeler decides whether the cluster centroid text belongs in any existing response class.
\begin{enumerate}
\item If centroid belongs in an existing group (most of the time): add the cluster to the existing response class.
\item Otherwise: create a new group with a memorable name, e.g “Greet + Pain Scale Question”.
\end{enumerate}
\end{enumerate}
We merge all responses that have the same impact on the user, and could therefore be used interchangeably. For example, even though “How long have you had the symptoms?” and “When did the symptoms start?” do not mean the same thing, they are both members of the same response class.

\end{enumerate}



==> sections/exp.old.tex <==

\subsection{Evaluation Criteria}
\label{eval_crit}

We train and validate on labeled (context, response) pairs, i.e pairs where the response is a member of a response class. All 187 response classes are present in both train and validation data.
Experiments that compare classification architectures on the same dataset measure validation accuracy: how often the classifier predicts the correct response class.

The test data is drawn randomly from (conversation, response) pairs that are not in the training data, so 91\% of test data responses are unlabeled. Given the low correlation of automated metrics such as BLEU score to human judgment of response quality reported in \citet{metrics}, a group of medical doctors evaluated the quality of generated responses on the test data. 
For a given conversational context, evaluators compared the doctor response observed in the data to a model's suggested response.  Evaluators reported whether a model's response is either (a) equivalent to the observed response, (b) different but worse, (c) different but equal quality, or (d) different but higher quality. For example, “Hoping for the best, take care.” and "Take care!!!!” would be marked equivalent.
Evaluators were prompted to consider the medical relevance of questions (e.g. marking down a response that asked a patient if they have nausea after the patient reported vomiting), and whether responses moved the conversation forward. They were not shown which model's output they were evaluating. The results are shown in Table \ref{qresults}.

\section{Results}
\begin{table}[!htbp]
\centering
\begin{tabular}{@{}lll@{}}
\toprule
                                & Generative & Discriminative \\ \midrule
a. Equivalent to Dr.                   & 56\%       & 71\%           \\
b. Different, higher quality & 1\%        & 6\%            \\
c. Different, equal quality  & 25\%        & 11\%           \\ 
d. Different, lower quality & 18\%        & \textbf{12\%}            \\ \bottomrule
\end{tabular}

\caption{We find that on 775 test set conversations, the discriminative model compares favorably to the generative model. Evaluators reported whether a model's response (a) equivalent to the observed response, (b) different but worse, (c) different but equal quality, or (d) different but higher quality. More details are explained in Section \ref{eval_crit}.}
\label{qresults}
\end{table}


\section{Experiments}

\textbf{How much context to use:} We find, somewhat counterintuitively, that the ULMFit classifier does not benefit from using more than the last 6 turns of conversation history, as shown in Table \ref{ctxtab}.

\begin{table}[!htbp]
\centering
\begin{tabular}{@{}llllllllllll@{}}
\toprule
Max Turns of History   & 1      & 2      & 3      & 4      & 5      & 6      & 7      & All   \\ \midrule
Validation Accuracy & 44.5\% & 53.3\% & 55.3\% & 56.7\% & 56.3\% & \textbf{57.7\%} & 57.4\% & 57.0\%  \\ \bottomrule
\end{tabular}

\caption{One turn is all messages sent consecutively by one conversation participant. Observations are truncated to the most recent $n$ turns.}
\label{ctxtab}
\end{table}

%Table 3: Other Architectures%

\begin{table}[!htbp]
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
Classifier          & 4 turn accuracy & 8 turn accuracy & Encoder Finetune Time & Train Time \\ \midrule
LSTM                & 49.30\%         & 49.20\%         & 0                     & 2h         \\
Hierarchical LSTM   & 47.80\%         & 49.40\%         & 0                     & 6h         \\
GPT2$^\dag$                & 56.64\%         & 56.82\%         & 12h                   & 6h         \\
ULMFit              & \textbf{56.70}\%         & \textbf{57.00}\%         & 12h                   & \textbf{40 mins}    \\
Hierarchical ULMFit & 53.80\%         & 54.90\%         & 12h                   & 18h        \\ \bottomrule
\end{tabular}

\caption{Architecture comparison: $^\dag$ Follows \citet{hface} and then adds classification training until convergence. Hierarchical models are described in detail in the Experiments section.}
\label{archtab}
\end{table}

\textbf{Hierarchical Encoding:} \citet{serban} explain their hierarchical setup, which \citet{airbnb} also use, nicely: “The encoder RNN encodes the tokens appearing within the utterance, and the context RNN encodes the temporal structure of the utterances appearing so far in the dialogue, allowing information and gradients to flow over longer time spans.” We tested two different utterance encoders: the pretrained AWD-LSTM language model, and a randomly initialized QRNN trained from scratch. In both settings, the context RNN was a randomly initialized QRNN. We found that ULMFit performed significantly better without hierarchy, while QRNN performed comparably. 
We attribute part of this discrepancy with previous work to the large variance in the length of each turn in our data. Turns vary from 2 to 304 tokens, after truncation, requiring large amounts of padding and smaller batch sizes. Hierarchical ULMFit on 8 turns could only be trained with batch size 32, while the flat ULMFit fits 512 examples in each batch.
\newline\textbf{GPT2:} We experimented with a modified version of HuggingFace’s ConvAI architecture, which won the 2019 PersonaChat competition. To make a fairer comparison, we start by following the authors procedure: finetune GPT2 weights on our conversation data with language modeling and multiple choice losses. We then discard the multiple choice head and language modeling heads, and and attach a one layer classification head to the finetuned transformer, which we train until convergence (5 epochs). This results in similar accuracy to the ULMFit architecture, as shown in Table 3, but is much more expensive computationally (10x train time, 20x slower inference) than ULMFit, and would have required significant modification to meet our latency requirements.
\newline\textbf{Opting Out:}
Since the discriminative model is only generated on (context, response) pairs from a fixed bank of responses, it will occasionally see context that does not match any of the responses it is trained on. In these circumstances, it should not suggest a reply to the doctor. If we restrict our evaluations to the responses where the discriminative model is more confident than average (as measured by the maximum predicted probability), the error rate falls from 11\% to 2\%.
%In situations where the discriminative model does not have high confidence, the generative model could take over.
\newline\textbf{Different Response Grouping Procedures:}
We compared our 187 response group approach described in the Approach section with two other approaches: one that used the same human labeling step but only generated 40 clusters, and another that eliminated the human in the loop and generated 897 clusters with KMeans. The results, shown in Table \ref{rset_ablation}, suggest that manually adding another 147 choices (from 40 to 187) to the response bank significantly improved the quality of suggested responses. Moreover, responses taken from clusters produced without human merging are less likely to be usable. 
%Table 4: Different Response Sets  (Metrics) %
\begin{table}[!htbp]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
\# Classes & \# Train Examples & \%Bad Responses & Unique per 100 responses \\ \midrule
40$^ \dag$        & 19,300     & 38.2\%            & 17                       \\
188$^ \dag$       & 72,981     & 11.1\%            & 28                       \\
879$^ \phi$       & 42,941     & 33.7\%            & 49                       \\ \bottomrule
\end{tabular}

\caption{$^\dag$ Generated with process described in Section 2, including manual merge step. $^\phi$ Generated with KMeans and no manual merging or review. \% Bad responses is calculated on 100 test set examples using the the manual evaluation process outlined above. Unique per 100 responses measures how many unique responses are generated per 100 conversation contexts, and is computed on 1000 test set suggestions.}
\label{rset_ablation}
\end{table}


==> sections/related.old.tex <==
\section{Related Work}
\citet{lit_review} survey conversational agents in healthcare and find 13 publications, the most advanced of which follow the dialogue state tracking pattern to generate templated or hard-coded content retrieved from a data structure.

\citet{fitz} propose Woebot, a conversational agent designed to deliver cognitive behavioral theraby in the form of brief conversations with users. Underlying Woebot is a decision tree, where each node has a piece of content to send to the user, and (for some nodes) a proprietary NLP system, to determine which node to send the user to based on their most recent reply. 

\citet{minutolo2017conversational} prototype a system for turning medical factoid questions into structured queries over a knowledge graph. The system covers a few example medical conditions, and asks the patient for more information until enough slots are filled to execute a valid query. Patient utterances must match a specific set of templates and synomyms to ensure correct queries.

\citet{ni2017mandy} present a patient intake chatbot focused on four diseases. "MANDY" asks users to confirm or deny possible symptoms, then uses a differential diagnosis algorithm to generate a most likely disease list. After enough questions have been asked to establish confidence, the hypothesis list is sent to a doctor.

Whereas healthcare dialogue systems tend to rely on external data structures and generate responses that cover a fixed set of user intents, recent "open-domain" conversational assistants require less external knowledge and can generate almost anything.

\citet{gmail} introduced the first neural suggested response system for Gmail. Their seq2seq (generative) approach, trained exclusively on historical email data, focuses exclusively on generating the “25\% of replies that have 20 tokens or less”.

\citet{airbnb}'s AirBNB customer service chatbot, also uses a discriminative approach, but does not attempt to cover the whole response space and differs architecturally. Whereas our approach restricts the output space to 187 responses that attempt to cover the whole output space, the AirBNB system chooses from 71 one sentence investigative questions, each representing a cluster of questions, and leaves other response types, like statements and courtesy questions, to a separate model. Although the authors do not report how much of their data these 71 clusters cover, we suspect that it is large, and that their conversations are more homogenous than ours, since our largest 71 clusters cover only 6\% of our data (15\% if we restrict to questions.) The authors also enforce that their clusters cover all "Issue Types", a field we do not collect.

More recently, \citet{hface} won the 2019 PersonaChat competition with "TransferTransfo", a generative transformer approach.
The model starts training with pretrained weights from the GPT2 transformer, then finetunes with the PersonaChat data on a combination of two loss functions: next-utterance classification loss and language modeling (next word prediction) loss. Each task is performed with an associated linear layer that consumes the final hidden state of the self-attention block of the transformer, and both losses are backpropogated into the original transformer. Generation is performed in a typical generative manner: beam search with sampling and a blacklist to prevent copying from old utterances.


==> sections/related_anitha.tex <==
\section{Related Work}


\par \noindent
\textbf{Healthcare dialog models:} Much of the work on dialog models in healthcare emphasize on generating templated content supported by knowledge graph of some form ({\it c.f.} \cite{lit_review} for a comprehensive survey).  In \citet{ni2017mandy}, a system for patient information gathering was introduced with the goal to ask users to confirm or deny possible symptoms from a knowledge graph of disease-finding relationships, so that a ranked list of potential diagnosis can be identified.  In \citet{minutolo2017conversational} , a slot-filling approach was presented for answering medical factoid questions; in this setting, users are progressively asked questions until enough slots are filled to create a valid query.  In \citet{fitz}, a decision tree of content related to cognitive behavior therapy was assumed to be available. Then, the conversational agent interacts with the user through brief conversations, by traversing the tree. 
Our work departs from this line of work in multiple dimensions: First, we do not assume access to an external knowledge base.  Second, we are interested in a full-fledged conversational interactions, as opposed to use of templates.  Third, we take a step towards building true conversational agent by enabling the machine learned models to be part of a doctor's workflow - suggest responses to doctors-in-the-loop.



%Whereas healthcare dialogue systems tend to rely on external data structures and generate responses that cover a fixed set of user intents, recent "open-domain" conversational assistants require less external knowledge and can generate almost anything.


\par \noindent
\textbf{Generative dialog models:}

\citet{gmail} introduced the first neural suggested response system for Gmail. Their seq2seq (generative) approach, trained exclusively on historical email data, focuses exclusively on generating the “25\% of replies that have 20 tokens or less”.

More recently, \citet{hface} won the 2019 PersonaChat competition with "TransferTransfo", a generative transformer approach.
The model starts training with pretrained weights from the GPT2 transformer, then finetunes with the PersonaChat data on a combination of two loss functions: next-utterance classification loss and language modeling (next word prediction) loss. Each task is performed with an associated linear layer that consumes the final hidden state of the self-attention block of the transformer, and both losses are backpropogated into the original transformer. Generation is performed in a typical generative manner: beam search with sampling and a blacklist to prevent copying from old utterances.

\par \noindent

\textbf{Discriminative models for dialog:}

The closest work to ours is that of AirBNB customer service chatbot \cite{airbnb} which also uses a discriminative approach. 

but does not attempt to cover the whole response space and differs architecturally. Whereas our approach restricts the output space to 187 responses that attempt to cover the whole output space, the AirBNB system chooses from 71 one sentence investigative questions, each representing a cluster of questions, and leaves other response types, like statements and courtesy questions, to a separate model. Although the authors do not report how much of their data these 71 clusters cover, we suspect that it is large, and that their conversations are more homogenous than ours, since our largest 71 clusters cover only 6\% of our data (15\% if we restrict to questions.) The authors also enforce that their clusters cover all "Issue Types", a field we do not collect.


